Rankify: A Comprehensive Python Toolkit for Retrieval, Re-Ranking, and Retrieval-Augmented Generation

Retrieval, re-ranking, and retrieval-augmented generation (RAG) are critical components of modern applications in information retrieval, question answering, or knowledge-based text generation. However, existing solutions are often fragmented, lacking a unified framework that easily integrates these essential processes. The absence of a standardized implementation, coupled with the complexity of retrieval and re-ranking workflows, makes it challenging for researchers to compare and evaluate different approaches in a consistent environment. While existing toolkits such as Rerankers and RankLLM provide general-purpose reranking pipelines, they often lack the flexibility required for fine-grained experimentation and benchmarking. In response to these challenges, we introduce Rankify, a powerful and modular open-source toolkit designed to unify retrieval, re-ranking, and RAG within a cohesive framework. Rankify supports a wide range of retrieval techniques, including dense and sparse retrievers, while incorporating state-of-the-art re-ranking models to enhance retrieval quality. Additionally, Rankify includes a collection of pre-retrieved datasets to facilitate benchmarking, available at Huggingface (https://huggingface.co/datasets/abdoelsayed/reranking-datasets-light). To encourage adoption and ease of integration, we provide comprehensive documentation (http://rankify.readthedocs.io/), an open-source implementation on GitHub (https://github.com/DataScienceUIBK/rankify), and a PyPI package for easy installation (https://pypi.org/project/rankify/). As a unified and lightweight framework, Rankify allows researchers and practitioners to advance retrieval and re-ranking methodologies while ensuring consistency, scalability, and ease of use.

==> table_bm25.tex <==

\begin{table*}[!ht]
\addtolength{\tabcolsep}{-0.65pt}
\small
\centering
\begin{tabular}{@{}l|cccccc|cccccc@{}}
\toprule
Retriever &  \multicolumn{6}{c}{NQ} & \multicolumn{6}{c}{WebQ}  \\

& Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100 & Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100 \\
\midrule
\multicolumn{11}{c}{\textit{Unsupervised Retrievers}} \\
\midrule
MSS         &  19.27 & 41.24 &  51.27 &  59.97 & 69.55  &  75.56 &  11.66 & 29.03 & 39.12  & 49.21 &  61.12 & 68.35\\

BM25        &  22.11 &  43.77 &  54.46 & 62.94  & 72.74  & 78.25    &  18.80  &  41.83 & 52.16  & 62.40 & 71.70 & 75.49\\


Contriever &  22.16 & 47.28 & 58.72 & 67.86 & 76.01 & 80.55 &  19.98 & 43.45 & 56.39  &65.69  & 74.85& 80.11\\




\midrule
\multicolumn{11}{c}{\textit{Supervised Retrievers}} \\
\midrule
DPR     & 48.67  &   68.78  &   74.54 &  79.19 & 83.71  & 85.70    &44.83   & 65.00 & 70.62  & 74.60 & 78.69 & 81.64\\


MSS-DPR    & 50.16 &  71.88  & 77.47 & 81.44 & 85.98 & 88.14 & 44.24  & 65.00 &  71.65 & 76.91 & 81.84 & 84.54\\

\midrule
\end{tabular}
\caption{ Top-K acc for retrievers
}
\label{tab:qa}
%\vspace{-6pt}
\end{table*}



\begin{table*}[!ht]
\addtolength{\tabcolsep}{-0.65pt}
\small
\centering
\begin{tabular}{@{}l | c c c c c c | c c c c c c@{}}\toprule
Retriever & \multicolumn{6}{c}{SQuAD-Open} & \multicolumn{6}{c}{TriviaQA}  \\

& Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100 & Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100  \\
\midrule
\multicolumn{11}{c}{\textit{Unsupervised Retrievers}} \\
\midrule
MSS         &  16.55 & 33.88 &  42.50 & 51.30 &  61.47 & 68.40  &  30.76 & 52.64 & 60.52  &67.17 & 74.57& 79.11\\



BM25        & 36.66  &   57.36 &  64.50 & 71.08  & 77.73  & 81.83    & 46.30  & 66.27 &  71.74 &  76.40 & 80.56 & 83.15 \\


Contriever &   20.80 &  44.30 & 54.65  & 63.39 & 72.82 &  78.20 & 34.16  & 59.48 &  68.00 &73.91  & 79.83& 82.93\\


\midrule
\multicolumn{11}{c}{\textit{Supervised Retrievers}} \\
\midrule
DPR     &  22.10 & 42.78 &  51.41 &  59.40 &  68.65 &  74.47   &     57.47 & 72.40 & 76.50  & 79.76 &  82.96 & 85.09 \\
MSS-DPR    &  32.52 &57.43 &  65.84 & 73.14  &  80.51 &  84.45    & 61.63  & 75.21 &  79.14  &81.85  & 84.92 &86.58 \\





\midrule
\end{tabular}
\caption{ Top-K acc for retrievers
}
\label{tab:qa2}
%\vspace{-6pt}
\end{table*}


\begin{table*}[!ht]
\addtolength{\tabcolsep}{-0.65pt}
\small
\centering
\begin{tabular}{@{}l | c c c c c c | c c c c c c@{}}\toprule
Retriever & \multicolumn{6}{c}{ArchivialQA} & \multicolumn{6}{c}{ChroniclingAmericaQA}  \\

& Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100 & Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100  \\
\midrule
\multicolumn{11}{c}{\textit{Unsupervised Retrievers}} \\
\midrule
%MSS         &   &     &   &   &   &     &   &  &   & & & \\
BM25        &  17.16 &  32.01   &  38.72 & 44.86  & 52.29  &57.58     & 4.18  & 11.23 &  15.82 &  20.86 & 27.48  & 32.47 \\



Contriever &  7.27 & 22.52  &  30.69 & 38.50  & 48.28 & 54.57 & 2.72&   9.86  &  15.05 & 20.21 & 27.25 & 32.65 \\
\midrule
\multicolumn{11}{c}{\textit{Supervised Retrievers}} \\
\midrule
DPR     & 16.75  &  30.21 &  36.53 &  42.79 &  50.55  &  56.08   & 5.70  &  14.91 &  20.10 &25.14 & 31.40& 36.24\\


%MSS-DPR    &   &     &   &   &   &     &   &  &   &  & &\\
\midrule
\end{tabular}
\caption{ Top-K acc for retrievers
}
\label{tab:qa3}
%\vspace{-6pt}
\end{table*}


\begin{table*}[!ht]
\addtolength{\tabcolsep}{-0.65pt}
\small
\centering
\begin{tabular}{@{}l | c c c c c c | c c c c c c@{}}\toprule
Retriever & \multicolumn{6}{c}{EntityQuestion} & \multicolumn{6}{c}{HotpotQA-Val}  \\

& Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100 & Top-1 & Top-5 &Top-10 & Top-20 &Top-50 & Top-100  \\
\midrule
\multicolumn{11}{c}{\textit{Unsupervised Retrievers}} \\
\midrule
%MSS         &   &     &   &   &   &     &   &  &   &  & &\\
BM25        &  43.35 & 60.50 & 66.07  & 70.61  & 75.40  &  79.05   & 27.27  & 44.09 &  50.70 & 56.54 & 64.09 & 69.29\\



Contriever &27.07 &47.99 &55.67 & 62.33 & 69.49 & 74.63 & 4.496  & 16.83 & 24.44  & 32.27 &41.40& 47.50 \\



\midrule
\multicolumn{11}{c}{\textit{Supervised Retrievers}} \\
\midrule
DPR     & 25.30  & 39.53  & 45.29  & 50.75  &  58.08 &  63.50   & 17.09  & 29.65 &  35.71 &42.16   &50.24 & 55.88\\


%MSS-DPR    &   &     &   &   &   &     &   &  &   & & & \\
\midrule
\end{tabular}
\caption{ Top-K acc for retrievers
}
\label{tab:qa4}
%\vspace{-6pt}
\end{table*}

==> tables/generator.tex <==

\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
  & \multicolumn{9}{c|}{\textbf{LLama V3 8B}} & \multicolumn{9}{c}{\textbf{LLama V3.1 8B}}\\

\multirow{3}{*}{\textbf{Retriever} }&\multicolumn{3}{c}{\textbf{NQ}} & \multicolumn{3}{c}{\textbf{TriviaQA}} & \multicolumn{3}{c|}{\textbf{WebQ}} & \multicolumn{3}{c}{\textbf{NQ}} & \multicolumn{3}{c}{\textbf{TriviaQA}} & \multicolumn{3}{c}{\textbf{WebQ}} \\

                      & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule
\multirow{1}{*}{BM25 } &          14.90  &  26.68  & 19.91  & 42.10 & 56.90 & 50.11 &  10.23 & 24.95 & 16.92 & 12.82 & 27.14 & 20.27 & 40.13 &58.40 &51.40 & 9.25 & 24.92 & 17.22 \\

\midrule
\multirow{1}{*}{MSS} &       12.82 & 22.96 & 17.36 & 31.90 &44.27  & 37.75 &  7.38 & 18.9 &11.81  & 11.19 & 23.37 & 17.81 & 30.74 & 45.82 &38.91 & 6.88 & 19.30 & 12.40\\






\midrule
\multirow{1}{*}{Contriever}   &      15.29  & 27.36 & 20.99 & 36.25 &  49.52 &  49.52 &  10.67 & 28.28 &  20.22 &13.24 & 27.68 &  21.88 &35.29  & 50.96 &44.19 & 9.35 &28.71 & 20.32\\






\midrule
\multirow{1}{*}{DPR}  &      28.08 & 45.40 & 36.37 & 45.88 & 61.24 & 54.58 &  19.83 & 40.27   & 30.98  & 23.21 & 44.99 & 36.03 &43.62 & 62.61& 55.97 & 14.32 & 38.27 &28.98 \\






\midrule
\multirow{1}{*}{MSS+DPR}&       28.17 & 46.72 & 37.00 &  47.69 & 63.66 & 57.08 &  13.92 &  40.87   & 30.57 & 23.68 & 46.70 &37.53 & 45.72 & 65.24 & 58.53 & 13.92 &38.97 & 29.67\\






\bottomrule
\end{tabular}
}
\caption{Zero-shot results of in-context learning on
The test set of NQ, TriviaQA, and WebQ uses the LLama 3/3.1 8B Model as RAG }
\label{tab:qa_LLama_3_3.1}
\end{table*}

\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
  & \multicolumn{9}{c|}{\textbf{Gemma-2-2b}} & \multicolumn{9}{c}{\textbf{Gemma-2-9b}}\\

\multirow{3}{*}{\textbf{Retriever} } & \multicolumn{3}{c}{\textbf{NQ}} & \multicolumn{3}{c}{\textbf{TriviaQA}} & \multicolumn{3}{c|}{\textbf{WebQ}} & \multicolumn{3}{c}{\textbf{NQ}} & \multicolumn{3}{c}{\textbf{TriviaQA}} & \multicolumn{3}{c}{\textbf{WebQ}} \\

&   EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule

\multirow{1}{*}{BM25 } &       14.02 & 25.55 & 18.53 & 43.28 & 52.78 & 47.01 & 14.71 & 37.74 & 27.21 & 19.81 & 26.95 & 22.05 & 57.55 & 65.53 & 60.29 & 14.96 & 24.87 & 20.13 \\






\midrule
\multirow{1}{*}{MSS} &      13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\






\midrule
\multirow{1}{*}{Contriever}   &        13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\


\midrule
\multirow{1}{*}{DPR}  &     13.99 & 25.44 & 18.53 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

\midrule
\multirow{1}{*}{MSS+DPR}&       13.96 & 25.41 & 18.50 & 33.05 & 42.24 & 36.23 & 14.71 & 37.74 & 27.21 & 19.78 & 26.86 & 22.08 & 50.93 & 58.57 & 53.28 & 14.96 & 24.92 & 20.18 \\

\bottomrule
\end{tabular}
}
\caption{
Zero-shot results of in-context learning on
The test set of NQ, TriviaQA, and WebQ uses the Gemma Model as RAG.
}
\label{tab:qa_Gemma}
\end{table*}
\begin{table*}[!ht]
%\addtolength{\tabcolsep}{-0.65pt}
%\small
\centering
\resizebox{1.0\textwidth}{!}{  % Resize the table to fit the page width
\setlength\tabcolsep{3pt}
\begin{tabular}{@{}l | ccc| ccc | ccc |ccc | ccc | ccc @{}}
\toprule
 &  \multicolumn{9}{c|}{\textbf{Llama-2-13b-hf}} & \multicolumn{9}{c}{\textbf{Mistral-7B-v0.1}}\\

\multirow{3}{*}{\textbf{Retriever} } & \multicolumn{3}{c}{\textbf{NQ}} & \multicolumn{3}{c}{\textbf{TriviaQA}} & \multicolumn{3}{c|}{\textbf{WebQ}} & \multicolumn{3}{c}{\textbf{NQ}} & \multicolumn{3}{c}{\textbf{TriviaQA}} & \multicolumn{3}{c}{\textbf{WebQ}} \\

&   EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con  & EM & Recall  & Con & EM & Recall  & Con & EM & Recall  & Con \\
\midrule

\multirow{1}{*}{BM25 } 
&        21.14 & 30.82 & 24.46 & 57.90 & 65.27 & 59.57 & 19.54 & 37.38 & 27.51 & 11.19 & 13.45 & 11.80 & 52.85 & 58.11 & 53.82 & 6.40 & 8.46 & 6.84 \\

\midrule
\multirow{1}{*}{MSS} 
&       21.52 & 30.92 & 24.18 & 51.75 & 58.58 & 53.35 & 20.62 & 39.45 & 29.68 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\


\midrule
\multirow{1}{*}{Contriever}   
&       20.47 & 30.13 & 23.85 & 42.69 & 47.12 & 43.40 & 19.98 & 37.74 & 27.61 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\


\midrule
\multirow{1}{*}{DPR}  
&     21.94 & 31.36 & 24.88 & 51.07 & 57.97 & 52.71 & 19.83 & 37.35 & 28.05 & 11.11 & 13.36 & 11.69 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\


\midrule
\multirow{1}{*}{MSS+DPR}
&       21.47 & 31.26 & 24.60 & 51.35 & 58.26 & 53.01 & 19.83 & 37.37 & 27.61 & 11.08 & 13.33 & 11.66 & 42.69 & 47.12 & 43.40 & 6.40 & 8.46 & 6.84 \\


\bottomrule
\end{tabular}
}
\caption{
Zero-shot results of in-context learning on
the test set of NQ, TriviaQA, and WebQ  using Llama-2-13b-hf and Mistral-7B-v0.1 as RAG
}
\label{tab:qa_Llama-2-13b}
\end{table*}

